Lifelong Language Knowledge Distillation

It is challenging to perform lifelong language learning (LLL) on a stream of different tasks without any performance degradation comparing to the multi-task counterparts. To address this issue, we present Lifelong Language Knowledge Distillation (L2KD), a simple but efficient method that can be easily applied to existing LLL architectures in order to mitigate the degradation. Specifically, when the LLL model is trained on a new task, we assign a teacher model to first learn the new task, and pass the knowledge to the LLL model via knowledge distillation. Therefore, the LLL model can better adapt to the new task while keeping the previously learned knowledge. Experiments show that the proposed L2KD consistently improves previous state-of-the-art models, and the degradation comparing to multi-task models in LLL tasks is well mitigated for both sequence generation and text classification tasks.

==> tables/TCanalysis.tex <==
\begin{table*}[bh!]
% \footnotesize
\centering
\small
\setlength\tabcolsep{3pt}
\begin{tabular}{lccccc|c}
\toprule
& amazon & yelp & yahoo & ag & dbpedia & Avg \\
\midrule

% Single$_\text{(QA)}$ & 55.9 & 63.3 & 70.6 & 93.6 & 99.0 & 76.5 \\
% Single$_\text{(QA+LM)}$ & 56.9 & \textbf{64.5} & 70.1 & 93.7 & \textbf{99.1} & 76.9 \\
% Multi$_\text{(QA)}$ & 56.6 & 63.3 & 69.2 & 93.7 & 99.0 & 76.4 \\
% Multi$_\text{(QA+LM)}$ & \textbf{57.8} & 64.4 & \textbf{70.9} & \textbf{94.0} & \textbf{99.1} & \textbf{77.2} \\

%  & amazon & yelp & yahoo & ag & dbpedia & Avg \\
Teacher Acc & 55.50 & 64.11 & 71.20 & 93.76 & 99.11 & 76.73 \\
\midrule
LAMOL Acc & 52.74 & 61.61 & 70.29 & 93.63 & 99.13 & 75.48 \\
Acc in group (A)/(B) & 36.75/15.99 & 48.61/13.00 & 62.86/7.43 & 91.09/2.54 & 98.89/0.24 & 67.64/7.84 \\
\midrule
+ Word-KD Acc & 57.54 & 63.59 & 71.28 & 93.91 & 99.24 & 77.11 \\
Acc in group (A)/(B) & 40.70/16.84 & 51.24/12.36 & 63.82/7.46 & 91.58/2.33 & 98.96/0.28 & 69.26/7.85 \\
diff to LAMOL & +3.95/+0.86 & +2.63/-0.64 & +0.96/+0.03 & +0.49/-0.21 & +0.07/+0.04 & +1.62/+0.01 \\
\midrule
+ Seq-KD$_\text{soft}$ Acc & 55.74 & 62.00 & 71.26 & 93.89 & 99.18 & 76.42 \\
Acc in group (A)/(B) & 39.08/16.66 & 49.68/12.32 & 63.64/7.62 & 91.71/2.18 & 98.96/0.22 & 68.62/7.80 \\
diff to LAMOL & +2.33/+0.67 & +1.08/-0.68 & +0.79/+0.18 & +0.62/-0.36 & +0.07/-0.01 & +0.98/-0.04 \\
\midrule
+ Seq-KD acc & 56.78 & 62.32 & 71.13 & 93.45 & 99.11 & 76.56 \\
Acc in group (A)/(B) & 39.95/16.83 & 49.87/12.45 & 63.74/7.39 & 91.09/2.36 & 98.93/0.17 & 68.72/7.84 \\
diff to LAMOL & +3.20/+0.84 & +1.26/-0.55 & +0.88/-0.04 & +0.00/-0.18 & +0.04/-0.07 & +1.08/+0.00 \\



\bottomrule
\end{tabular}
\caption{The accuracy in the group (A) and (B) detailed in five classification datasets.}
\label{tab:tcanalysis}
\end{table*}



% 可能改用圖表呈現

% \begin{table}[t!]
% \footnotesize
% \centering
% % \small
% \setlength\tabcolsep{3pt}
% \begin{tabular}{lccccc|c}
% \toprule
% & amazon & yelp & yahoo & ag & dbpedia & Avg \\
% \midrule

% Teacher Acc & 55.50 & 64.11 & 71.20 & 93.76 & 99.11 & 76.73 \\
% \midrule
% LAMOL Acc & 52.74 & 61.61 & 70.29 & 93.63 & 99.13 & 75.48 \\
% Acc split in (A) & 36.75 & 48.61 & 62.86 & 91.09 & 98.89 & 67.64 \\
% Acc split in (B) & 15.99 & 13.00 & 7.43 & 2.54 & 0.24 & 7.84 \\
% \midrule
% + Word-KD Acc & 57.54 & 63.59 & 71.28 & 93.91 & 99.24 & 77.11 \\
% Acc split in (A) & 40.70 & 51.24 & 63.82 & 91.58 & 98.96 & 69.26 \\
% diff to LAMOL & +3.95 & +2.63 & +0.96 & +0.49 & +0.07 & +1.62 \\
% Acc split in (B) & 16.84 & 12.36 & 7.46 & 2.33 & 0.28 & 7.85 \\
% diff to LAMOL & +0.86 & -0.64 & +0.03 & -0.21 & +0.04 & +0.01 \\
% \midrule
% + Seq-KD$_\text{soft}$ Acc & 55.74 & 62.00 & 71.26 & 93.89 & 99.18 & 76.42 \\
% Acc split in (A) & 39.08 & 49.68 & 63.64 & 91.71 & 98.96 & 68.62 \\
% diff to LAMOL & +2.33 & +1.08 & +0.79 & +0.62 & +0.07 & +0.98 \\
% Acc split in (B) & 16.66 & 12.32 & 7.62 & 2.18 & 0.22 & 7.80 \\
% diff to LAMOL & +0.67 & -0.68 & +0.18 & -0.36 & -0.01 & -0.04 \\
% \midrule
% + Seq-KD acc & 56.78 & 62.32 & 71.13 & 93.45 & 99.11 & 76.56 \\
% Acc split in (A) & 39.95 & 49.87 & 63.74 & 91.09 & 98.93 & 68.72 \\
% diff to LAMOL & +3.20 & +1.26 & +0.88 & +0.00 & +0.04 & +1.08 \\
% Acc split in (B) & 16.83 & 12.45 & 7.39 & 2.36 & 0.17 & 7.84 \\
% diff to LAMOL & +0.84 & -0.55 & -0.04 & -0.18 & -0.07 & +0.00 \\



% \bottomrule
% \end{tabular}
% \caption{Analysis on which group improves more on classification datasets.}
% \label{tab:tcanalysis}
% \end{table}

==> tables/TCsmall.tex <==
\begin{table}[ht]
\footnotesize
\centering
\caption{Experimental results on five text classification datasets.}
\label{tab:tc}
\footnotesize
\setlength\tabcolsep{3pt}

\begin{tabular}{lccccc|c}
\toprule
\textbf{Method} & amazon & yelp & yahoo & ag & dbpedia & Average \\
\midrule

Single$_\text{(QA)}$ & 55.5 & 60.4 & 69.1 & 91.6 & \textbf{98.7} & 75.1 \\
Single$_\text{(QA+LM)}$ & \textbf{56.8} & \textbf{60.9} & \textbf{69.7} & \textbf{92.0} & \textbf{98.7} & \textbf{75.6} \\
Multi$_\text{(QA)}$ & 54.3 & 59.2 & 66.6 & 90.6 & 98.2 & 73.8 \\
Multi$_\text{(QA+LM)}$ & 55.1 & 59.6 & 66.2 & 91.1 & 98.4 & 74.1 \\

\midrule
\multicolumn{7}{l}{\textbf{Left-to-right}}\\
\midrule
LAMOL & 51.1 & 57.6 & 66.4 & \textbf{91.1} & \textbf{98.8} & 73.0 \\
+ Word-KD & 53.5 & 56.4 & 66.4 & 90.3 & \textbf{98.8} & 73.1 \\
+ Seq-KD$_\text{soft}$ & 54.0 & 57.6 & 63.4 & 90.0 & \textbf{98.8} & 72.7 \\
+ Seq-KD & \textbf{54.8} & \textbf{57.9} & \textbf{66.6} & 90.4 & 98.7 & \textbf{73.7} \\

\midrule
\multicolumn{7}{l}{\textbf{Right-to-left}}\\
\midrule
LAMOL & 57.0 & 60.4 & 67.1 & 89.1 & 97.8 & 74.3 \\
+ Word-KD & \textbf{58.4} & \textbf{61.2} & 62.6 & \textbf{89.9} & \textbf{98.3} & 74.1 \\
+ Seq-KD$_\text{soft}$ & 57.8 & 60.6 & 65.4 & 88.9 & 98.2 & 74.2 \\
+ Seq-KD & 58.1 & \textbf{61.2} & \textbf{68.9} & 89.3 & \textbf{98.3} & \textbf{75.2} \\

\bottomrule
\end{tabular}
\end{table}

==> tables/tmp.tex <==

\begin{table}[t!]
%\footnotesize
% \small
\centering
\setlength\tabcolsep{3pt}
\begin{tabular}{clccc|c}
\toprule
\multicolumn{2}{l}{\textit{Non-Lifelong Methods}} & \bf WOZ & \bf CNN & \bf SQL & \bf Avg \\
\midrule
% Single-Task (QA) & 82.2 & 25.9 & 63.7 & 54.1 \\
(1)&Single QA & 84.8 & 25.5 & 63.1 & \textbf{57.8} \\
(2)&Single QA+LM & 82.2 & 25.9 & \textbf{63.7} & 54.1 \\
(3)&Multi$_{\text{same}}$ QA & 66.2 & 25.6 & 53.0 & 48.3 \\
(4)&Multi$_{\text{same}}$ QA+LM & 59.0 & 26.3 & 53.6 & 46.3 \\
(5)&Multi$_{\text{long}}$ QA & 82.7 & 26.1 & 61.1 & 56.6 \\
% (6)&Multi$_{\text{long}}$ QA+LM & 82.5 & \textbf{26.5} & 61.4 & 56.8 \\
(6)&Multi$_{\text{long}}$ QA+LM & \bf 85.4 & \bf 26.7 & 61.3 & \bf 57.8 \\
\midrule
% \hline
(7)& (6) + Seq-KD & 84.4 & 27.6 & 61.8 & 58.0 \\
\midrule
\multicolumn{5}{l}{\textit{Lifelong Methods (averaged over six orders)}} \\
\midrule
(a)&Finetune & 28.9 & 19.5 & 21.7 & 23.4 \\
(b)&LAMOL & 77.7 & 27.0 & 60.0 & 54.9 \\
(c)&(b)+Word-KD & 81.9 & 27.0 & \textbf{61.9} & 57.0 \\
(d)&(b)+Seq-KD$_{\text{soft}}$ & \textbf{82.6} & 26.9 & 61.7 & \textbf{57.1} \\
(e)&(b)+Seq-KD & 80.9 & \textbf{28.0} & 60.6 & 56.5 \\
\midrule
\multicolumn{5}{l}{\textit{STD of Lifelong Methods}} \\
\midrule
(f)&Finetune & 43.3 & 9.6 & 32.9 & 28.6 \\
(g)&LAMOL & 6.0 & \textbf{0.7} & 3.2 & 3.3 \\
(h)&(b)+Word-KD & 2.7 & \textbf{0.7} & \textbf{2.8} & 2.1 \\
(i)&(b)+Seq-KD$_{\text{soft}}$ & \textbf{1.8} & 1.0 & 3.0 & \textbf{1.9} \\
(j)&(b)+Seq-KD & 3.4 & 0.9 & 3.1 & 2.5 \\

\bottomrule
\end{tabular}
\caption{Averaged results at the end of the lifelong learning procedures over six orders, comparing to single task and multitask upper bound. The bold numbers are the best in the group.}
\label{tab:average}
\end{table}
